DeWave: Discrete EEG Waves Encoding for Brain Dynamics to Text Translation

The translation of brain dynamics into natural language is pivotal for brain-computer interfaces (BCIs). With the swift advancement of large language models, such as ChatGPT, the need to bridge the gap between the brain and languages becomes increasingly pressing. Current methods, however, require eye-tracking fixations or event markers to segment brain dynamics into word-level features, which can restrict the practical application of these systems. To tackle these issues, we introduce a novel framework, DeWave, that integrates discrete encoding sequences into open-vocabulary EEG-to-text translation tasks. DeWave uses a quantized variational encoder to derive discrete codex encoding and align it with pre-trained language models. This discrete codex representation brings forth two advantages: 1) it realizes translation on raw waves without marker by introducing text-EEG contrastive alignment training, and 2) it alleviates the interference caused by individual differences in EEG waves through an invariant discrete codex with or without markers. Our model surpasses the previous baseline (40.1 and 31.7) by 3.06% and 6.34%, respectively, achieving 41.35 BLEU-1 and 33.71 Rouge-F on the ZuCo Dataset. This work is the first to facilitate the translation of entire EEG signal periods without word-level order markers (e.g., eye fixations), scoring 20.5 BLEU-1 and 29.5 Rouge-1 on the ZuCo Dataset.

==> text/subject_wise_metric.tex <==
\begin{table*}[hbpt]
\caption{Evaluation metrics on subjects. The subject to be tested is removed from training, where the column name is the subject name. The test sample of each subject is quite limited with the same text ground truth, thus the numerical value of several subjects is the same.\label{tb:subjectwise}}
\small
\centering
\resizebox{1\textwidth}{!}{
\begin{tabular}{llllllllllllll}
\toprule
\textbf{Subject} & \textbf{YLS} & \textbf{YFS} & \textbf{YRH} & \textbf{YFR} &\textbf{ YAC} & \textbf{YSL} & \textbf{YAK} & \textbf{YMS }& \textbf{YSD} & \textbf{YHS} & \textbf{YDR} & \textbf{YRK }& \textbf{YIS} \\ \midrule
\textbf{BLEU-1} ~($\%$) & 43.37 & 43.11 & 43.37 & 42.21 & 43.08 & 43.43 & 43.37 & 43.37 & 43.37 & 43.27 & 43.50 & 43.37 & 43.37 \\
\textbf{BLEU-2}~($\%$) & 26.81 & 27.12 & 26.81 & 25.54 & 26.30 & 27.01 & 26.81 & 26.81 & 26.81 & 26.58 & 26.94 & 26.81 & 26.81 \\
\textbf{BLEU-3} ~($\%$)& 15.90 & 16.26 & 15.90 & 14.91 & 15.53 & 16.05 & 15.90 & 15.90 & 15.90 & 15.75 & 16.06 & 15.90 & 15.90 \\
\textbf{BLEU-4}~($\%$)& 9.46 & 9.77 & 9.46 & 8.43 & 9.17 & 9.61 & 9.46 & 9.46 & 9.46 & 9.23 & 9.63 & 9.46 & 9.46 \\
\textbf{ROUGE-R}~($\%$) & 33.04 & 32.61 & 33.04 & 31.81 & 32.76 & 33.35 & 33.04 & 33.04 & 33.04 & 32.90 & 33.12 & 33.04 & 33.04 \\
\textbf{ROUGE-P} ~($\%$)& 41.26 & 41.14 & 41.26 & 39.04 & 40.81 & 41.62 & 41.26 & 41.26 & 41.26 & 41.05 & 41.09 & 41.26 & 41.26 \\
\textbf{ROUGE-F} ~($\%$)& 36.62 & 36.32 & 36.62 & 35.00 & 36.28 & 36.95 & 36.62 & 36.62 & 36.62 & 36.41 & 36.61 & 36.62 & 36.62 \\ \bottomrule
\end{tabular}
}
\end{table*}

==> text/tableap_clip.tex <==
\begin{table}[h]
\vspace{-8pt}
\centering
\caption{\footnotesize \label{tb:scoreap} Extensive experimental comparison with SSL methods.}
\small
\vspace{-10pt}
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{cllllllll}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Eye}\\ \textbf{}\end{tabular}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{BLEU-N} ($\%$)}                                      & \multicolumn{3}{c}{\textbf{ROUGE-1} ($\%$)}                                           \\ \cline{3-9}
&                         & \multicolumn{1}{c}{N=1} & \multicolumn{1}{c}{N=2} & \multicolumn{1}{c}{N=3} & \multicolumn{1}{c}{N=4} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{F} \\ \hline
% $\checkmark$& Baseline           & 40.12                   & 23.18                   & 12.61                   & 6.80                    & \textbf{28.84}        & 31.69                 & 30.10                 \\
% $\checkmark$& BENDR           & 41.08                   & 23.87                   & 13.04                  & 7.26                    & {28.75}        & 31.36                 & 30.22                 \\
% $\checkmark$ & DeWave                  & \textbf{41.35}          & \textbf{24.15}          & \textbf{13.92}          & \textbf{8.22}           & 28.82                 & \textbf{33.71}        & \textbf{30.69}        \\ \hline
$\times$& Baseline$^T$        & 13.07                   & 5.78                    & 2.55                    & 1.10                    & 15.22                 & 18.08                 & 16.36                 \\
$\times$& SCL~\cite{jiang2021self}        & 16.65                   & 8.24                    & 3.85                   & 2.01                    & 18.56                 & 22.16                 & 19.05                 \\
$\times$& Wave2Vec        & 18.15                   & 8.94                   & 3.89                 & 2.04                    & 18.96                & 23.86               & 20.07                \\
$\times$& BENDR~\cite{kostas2021bendr}        & 18.48                   & 9.16                    & 4.05                  & 2.15                    & 19.03                & 25.22                & 21.18                \\
$\times$& DeWave                  & \textbf{20.51}          & \textbf{10.18}          & \textbf{5.16}           & \textbf{2.52}           & \textbf{21.18}        & \textbf{29.42}        & \textbf{24.27}        \\ 
$\times$& DeWave+CL                  & \textbf{21.09}          & \textbf{10.69}          & \textbf{5.88}           & \textbf{3.04}           & \textbf{22.01}        & \textbf{29.95}        & \textbf{24.68}        \\ 
\bottomrule
\end{tabular}
}
\vspace{-9pt}
\end{table}

==> text/tableap_cross.tex <==
\begin{table}[hbpt]
\vspace{-12pt}
\centering
\caption{\label{tb:crossap} Cross-subject performance average decreasing comparison on 18 human subjects, where MAML denotes the method with MAML training. The metric is the lower the better.}
%\vspace{-10pt}
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{clcccccccc}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Calib Data}\end{tabular}}& \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Method}\end{tabular}}& \multicolumn{4}{c}{\textbf{Eye fixation} $-\Delta (\%)$ $\downarrow$} & \multicolumn{4}{c}{\textbf{Raw EEG waves} $-\Delta (\%)$ $\downarrow$} \\ \cline{3-10} 
& & B-2 & B-4 & R-P & R-F & B-2 & B-4 & R-P & R-F \\ \hline
$\times$ &Baseline & 3.38 & 2.08 & 2.14 & 2.80 & 7.94 & 5.38 & 6.02 & 5.89 \\
$\checkmark$&Baseline+MAML~\cite{finn2017model} & 2.51 & 1.43 & \textbf{1.08} & 1.23 & 6.86 & 4.22 & 4.08 & 4.79 \\
$\times$&DeWave & {2.35} & \textbf{1.25} & 1.16 & \textbf{1.17} & \textbf{6.24} & \textbf{3.88} & \textbf{3.94} & \textbf{4.28} \\
$\checkmark$&DeWave+MAML~\cite{finn2017model} & \textbf{2.08} & \textbf{1.25} & 1.16 & \textbf{1.17} & \textbf{6.24} & \textbf{3.88} & \textbf{3.94} & \textbf{4.28} \\ \bottomrule
\end{tabular}
}
\vspace{-12pt}
\end{table}
